Bidirectional Decoding: Improving Action Chunking via Guided Test-Time Sampling

Predicting and executing a sequence of actions without intermediate replanning, known as action chunking, is increasingly used in robot learning from human demonstrations. Yet, its effects on the learned policy remain inconsistent: some studies find it crucial for achieving strong results, while others observe decreased performance. In this paper, we first dissect how action chunking impacts the divergence between a learner and a demonstrator. We find that action chunking allows the learner to better capture the temporal dependencies in demonstrations but at the cost of reduced reactivity to unexpected states. To address this tradeoff, we propose Bidirectional Decoding (BID), a test-time inference algorithm that bridges action chunking with closed-loop adaptation. At each timestep, BID samples multiple candidate predictions and searches for the optimal one based on two criteria: (i) backward coherence, which favors samples that align with previous decisions; (ii) forward contrast, which seeks samples of high likelihood for future plans. By coupling decisions within and across action chunks, BID promotes both long-term consistency and short-term reactivity. Experimental results show that our method boosts the performance of two state-of-the-art generative policies across seven simulation benchmarks and two real-world tasks. Code and videos are available at https://bid-robot.github.io.

==> figures/distribution.tex <==
\begin{tikzpicture}[scale=1.5]

% Draw Gaussian curves
\draw[thick, smooth, green!70!black, name path=demo1] plot[domain=-3:-1.3] (\x, {exp(-((\x+2)^2)/0.5)});
\draw[thick, smooth, green!70!black, name path=demo2] plot[domain=2.3:4] (\x, {exp(-((\x-3.2)^2)/0.5)});
\draw[thick, smooth, blue!70!black, name path=long] plot[domain=-1:1] (\x, {exp(-((\x)^2)/0.5)});
\draw[thick, smooth, red!70!black, name path=short] plot[domain=1.5:3.5] (\x, {exp(-((\x-2.5)^2)/0.5)});

% Draw x-axis
\draw[thick] (-3,0) -- (4,0) node[right] {};

% Plot points (markers) for previous decisions, short-horizon plans, long-horizon plans
\foreach \x in {-2, 2.2} \node[star,star points=6,fill=blue!70!black,scale=0.8] at (\x, 0) {};
\foreach \x in {1.8, 2.2, 2.6, 3, 3.4} \node[cross out,fill=red!70!black,scale=0.8] at (\x, 0) {};
\foreach \x in {-1.2, -0.8, -0.4, 0, 0.4, 0.8, 1.2} \node[cross out,fill=blue!70!black,scale=0.8] at (\x, 0) {};

% Arrow at the end
\draw[-{Stealth[length=2mm]}, thick] (4.1, 0) -- (4.5, 0);

% Legend
\begin{scope}[shift={(5.5,-0.5)}]
  \node[star,star points=6,fill=blue!70!black,scale=0.8, label=right:previous decision] at (0, 1.5) {};
  \node[cross out,fill=red!70!black,scale=0.8, label=right:short-horizon plans] at (0, 1) {};
  \node[cross out,fill=blue!70!black,scale=0.8, label=right:long-horizon plans] at (0, 0.5) {};
  \draw[thick, green!70!black] (0, 0) -- ++(1,0) node[right=2pt,black]{demo distribution};
\end{scope}

\end{tikzpicture}


==> figures/horizon.tex <==
\begin{tikzpicture}

% Style for the gradients
\definecolor{grayleft}{RGB}{250,250,250}
\definecolor{grayright}{RGB}{110,110,110}

% Legend above the figure

\node[draw,rectangle,minimum width=0.2cm,minimum height=0.2cm,fill=white] (white) at (-1.0,3.95) {}; % Adjusted y position for spacing
\node[right=0.02cm of white,font=\tiny] {Unknown};

\node[draw,rectangle,minimum width=0.2cm,minimum height=0.2cm,shade,left color=grayleft, right color=grayright] (gray) at (0.6,3.95) {}; % Adjusted x position for spacing
\node[right=0.02cm of gray,font=\tiny] {Known Context};

\node[draw,rectangle,minimum width=0.2cm,minimum height=0.2cm,pattern=north east lines, pattern color=gray] (hatched) at (2.65,3.95) {};
\node[right=0.02cm of hatched,font=\tiny] {Known Prediction};

% Main figure code

% Define the total length as a variable
\def\totallength{4.5}

% Define the block height
\def\blockheight{0.5}

% Define the lengths of the white, gray, and hatched parts for each row
\def\whitetop{0}
\def\graytop{4}
\def\hatchedtop{0.5}

\def\whitemid{2.5}
\def\graymid{0.75}
\def\hatchedmid{1.25}

\def\whitebottom{1}
\def\graybottom{0.75}
\def\hatchedbottom{2.75}

% Define the horizontal spacing between the text nodes and the blocks
\def\textspacing{-0.05} % Adjust this value to reduce the left margin

% Line width for borders
\def\linewidth{0.2mm}

% Pattern scaling for sparser hatching
\def\hatchscale{1}


% Top row
\shade[left color=grayleft, right color=grayright] (0, 3) rectangle (\graytop,\blockheight+3);
\fill[pattern=north east lines, pattern color=gray, scale=\hatchscale] (\graytop, 3) rectangle (\totallength,\blockheight+3);
\draw[black, line width=\linewidth] (0, 3) rectangle (\totallength,\blockheight+3); % Consistent border
\draw[black, line width=\linewidth] (0, 3) rectangle (\graytop,\blockheight+3); % Border for the gray block
\draw[black, line width=\linewidth] (\graytop, 3) rectangle (\totallength,\blockheight+3); % Border for the hatched block
\node[left, font=\tiny] at (\textspacing, 3.25) {$\pi_{(k,1)}^*$};

% Middle row
\shade[left color=grayleft, right color=grayright] (0, 2.2) rectangle (\graytop,\blockheight+2.2);
% Overlay the white part
\fill[white] (0, 2.2) rectangle (\whitemid,\blockheight+2.2);
% Overlay the hatched part with white fill first
\fill[white] (\whitemid+\graymid, 2.2) rectangle (\totallength,\blockheight+2.2);
\fill[pattern=north east lines, pattern color=gray, scale=\hatchscale] (\whitemid+\graymid, 2.2) rectangle (\totallength,\blockheight+2.2);
\draw[black, line width=\linewidth] (0, 2.2) rectangle (\totallength,\blockheight+2.2); % Consistent border
\draw[black, line width=\linewidth] (0, 2.2) rectangle (\whitemid,\blockheight+2.2); % Border for the white block
\draw[black, line width=\linewidth] (\whitemid, 2.2) rectangle (\whitemid+\graymid,\blockheight+2.2); % Border for the gray block
\draw[black, line width=\linewidth] (\whitemid+\graymid, 2.2) rectangle (\totallength,\blockheight+2.2); % Border for the hatched block
\node[left, font=\tiny] at (\textspacing, 2.45) {$\pi_{(c,h)}$};

% Bottom row
\shade[left color=grayleft, right color=grayright] (0, 1.4) rectangle (\graytop,\blockheight+1.4);
% Overlay the white part
\fill[white] (0, 1.4) rectangle (\whitebottom,\blockheight+1.4);
% Overlay the hatched part with white fill first
\fill[white] (\whitebottom+\graybottom, 1.4) rectangle (\totallength,\blockheight+1.4);
\fill[pattern=north east lines, pattern color=gray, scale=\hatchscale] (\whitebottom+\graybottom, 1.4) rectangle (\totallength,\blockheight+1.4);
\draw[black, line width=\linewidth] (0, 1.4) rectangle (\totallength,\blockheight+1.4); % Consistent border
\draw[black, line width=\linewidth] (0, 1.4) rectangle (\whitebottom,\blockheight+1.4); % Border for the white block
\draw[black, line width=\linewidth] (\whitebottom, 1.4) rectangle (\whitebottom+\graybottom,\blockheight+1.4); % Border for the gray block
\draw[black, line width=\linewidth] (\whitebottom+\graybottom, 1.4) rectangle (\totallength,\blockheight+1.4); % Border for the hatched block
\node[left, font=\tiny] at (\textspacing, 1.65) {$\pi_{(c,h+d)}$};

\end{tikzpicture}


==> figures/latent.tex <==
% \begin{tikzpicture}[
%     nodeSize/.style={minimum size=1cm}, % Node diameter
%     horizontalSpacing/.style={node distance=2cm and 1.5cm}, % Horizontal spacing
%     verticalSpacing/.style={node distance=2cm and 1cm}, % Vertical spacing
%     edgeThickness/.style={line width=1pt}, % Edge thickness
%     stateColor/.style={circle, draw, minimum size=1cm, thick, fill=white}, % State node color
%     actionColor/.style={circle, draw, minimum size=1cm, thick, fill=white}, % Action node color
%     auxiliaryColor/.style={circle, draw, minimum size=1cm, thick, fill=gray!20}, % Auxiliary node color
%     goalColor/.style={circle, draw, minimum size=1cm, thick, fill=blue!20}, % Goal node color
%     auxiliaryEdgeColor/.style={gray, thick}, % Auxiliary edge color
%     goalEdgeColor/.style={blue, thick}, % Goal edge color
% ]

% % Nodes
% \node[stateColor, nodeSize] (s0) {$s_0$};
% \node[stateColor, nodeSize, right=of s0, horizontalSpacing] (s1) {$s_1$};
% \node[stateColor, nodeSize, right=of s1, horizontalSpacing] (s2) {$s_2$};
% \node[stateColor, nodeSize, right=of s2, horizontalSpacing] (s3) {$s_3$};
% \node[stateColor, nodeSize, right=of s3, horizontalSpacing] (s4) {$s_4$};
% \node[stateColor, nodeSize, right=of s4, horizontalSpacing] (s5) {$s_5$};
% \node[stateColor, nodeSize, right=of s5, horizontalSpacing] (s6) {$s_6$};
% \node[stateColor, nodeSize, right=of s6, horizontalSpacing] (s7) {$s_7$};
% \node[stateColor, nodeSize, right=of s7, horizontalSpacing] (s8) {$s_8$};

% \node[actionColor, nodeSize, below=of s0, verticalSpacing] (a1) {$a_1$};
% \node[actionColor, nodeSize, below=of s1, verticalSpacing] (a2) {$a_2$};
% \node[actionColor, nodeSize, below=of s2, verticalSpacing] (a3) {$a_3$};
% \node[actionColor, nodeSize, below=of s3, verticalSpacing] (a4) {$a_4$};
% \node[actionColor, nodeSize, below=of s4, verticalSpacing] (a5) {$a_5$};
% \node[actionColor, nodeSize, below=of s5, verticalSpacing] (a6) {$a_6$};
% \node[actionColor, nodeSize, below=of s6, verticalSpacing] (a7) {$a_7$};
% \node[actionColor, nodeSize, below=of s7, verticalSpacing] (a8) {$a_8$};

% \node[auxiliaryColor, below right=of a2, verticalSpacing] (z1) {$z_{1:4}$};
% \node[auxiliaryColor, below right=of a6, verticalSpacing] (z2) {$z_{5:8}$};
% \node[goalColor, nodeSize, below right= of z1] (zg) {$z_g$};



% % Edges
% \draw[->, edgeThickness] (s0) -- (s1);
% \draw[->, edgeThickness] (s1) -- (s2);
% \draw[->, edgeThickness] (s2) -- (s3);
% \draw[->, edgeThickness] (s3) -- (s4);
% \draw[->, edgeThickness] (s4) -- (s5);
% \draw[->, edgeThickness] (s5) -- (s6);
% \draw[->, edgeThickness] (s6) -- (s7);
% \draw[->, edgeThickness] (s7) -- (s8);

% \draw[->, edgeThickness] (a1) -- (s1);
% \draw[->, edgeThickness] (a2) -- (s2);
% \draw[->, edgeThickness] (a3) -- (s3);
% \draw[->, edgeThickness] (a4) -- (s4);
% \draw[->, edgeThickness] (a5) -- (s5);
% \draw[->, edgeThickness] (a6) -- (s6);
% \draw[->, edgeThickness] (a7) -- (s7);
% \draw[->, edgeThickness] (a8) -- (s8);

% \draw[->, edgeThickness] (s0) -- (a1);
% \draw[->, edgeThickness] (s1) -- (a2);
% \draw[->, edgeThickness] (s2) -- (a3);
% \draw[->, edgeThickness] (s3) -- (a4);
% \draw[->, edgeThickness] (s4) -- (a5);
% \draw[->, edgeThickness] (s5) -- (a6);
% \draw[->, edgeThickness] (s6) -- (a7);
% \draw[->, edgeThickness] (s7) -- (a8);

% \draw[->, auxiliaryEdgeColor] (z1) -- (a1);
% \draw[->, auxiliaryEdgeColor] (z1) -- (a2);
% \draw[->, auxiliaryEdgeColor] (z1) -- (a3);
% \draw[->, auxiliaryEdgeColor] (z1) -- (a4);

% \draw[->, auxiliaryEdgeColor] (z2) -- (a5);
% \draw[->, auxiliaryEdgeColor] (z2) -- (a6);
% \draw[->, auxiliaryEdgeColor] (z2) -- (a7);
% \draw[->, auxiliaryEdgeColor] (z2) -- (a8);

% \draw[->, goalEdgeColor] (zg) -- (z1);
% \draw[->, goalEdgeColor] (zg) -- (z2);

% \end{tikzpicture}



% Slightly smaller size of the same diagram

\begin{tikzpicture}[
    nodeSize/.style={minimum size=0.3cm}, % Node diameter
    horizontalSpacing/.style={node distance=0.5cm and 0.5cm}, % Horizontal spacing
    verticalSpacing/.style={node distance=0.5cm and 0.5cm}, % Vertical spacing
    edgeThickness/.style={line width=0.5pt}, % Edge thickness
    stateColor/.style={circle, draw, minimum size=0.3cm, thick, fill=white}, % State node color
    actionColor/.style={circle, draw, minimum size=0.3cm, thick, fill=white}, % Action node color
    auxiliaryColor/.style={circle, draw, minimum size=0.3cm, thick, fill=gray!20}, % Auxiliary node color
    goalColor/.style={circle, draw, minimum size=0.3cm, thick, fill=blue!20}, % Goal node color
    auxiliaryEdgeColor/.style={gray, thick}, % Auxiliary edge color
    goalEdgeColor/.style={blue, thick}, % Goal edge color
]

% Nodes
\node[stateColor, nodeSize] (s0) {$s_0$};
\node[stateColor, nodeSize, right=of s0, horizontalSpacing] (s1) {$s_1$};
\node[stateColor, nodeSize, right=of s1, horizontalSpacing] (s2) {$s_2$};
\node[stateColor, nodeSize, right=of s2, horizontalSpacing] (s3) {$s_3$};
\node[stateColor, nodeSize, right=of s3, horizontalSpacing] (s4) {$s_4$};
\node[stateColor, nodeSize, right=of s4, horizontalSpacing] (s5) {$s_5$};
\node[stateColor, nodeSize, right=of s5, horizontalSpacing] (s6) {$s_6$};
\node[stateColor, nodeSize, right=of s6, horizontalSpacing] (s7) {$s_7$};
\node[stateColor, nodeSize, right=of s7, horizontalSpacing] (s8) {$s_8$};

\node[actionColor, nodeSize, below=of s0, verticalSpacing] (a1) {$a_1$};
\node[actionColor, nodeSize, below=of s1, verticalSpacing] (a2) {$a_2$};
\node[actionColor, nodeSize, below=of s2, verticalSpacing] (a3) {$a_3$};
\node[actionColor, nodeSize, below=of s3, verticalSpacing] (a4) {$a_4$};
\node[actionColor, nodeSize, below=of s4, verticalSpacing] (a5) {$a_5$};
\node[actionColor, nodeSize, below=of s5, verticalSpacing] (a6) {$a_6$};
\node[actionColor, nodeSize, below=of s6, verticalSpacing] (a7) {$a_7$};
\node[actionColor, nodeSize, below=of s7, verticalSpacing] (a8) {$a_8$};

\node[auxiliaryColor, below right=of a2, verticalSpacing] (z1) {$z_{1:4}$};
\node[auxiliaryColor, below right=of a6, verticalSpacing] (z2) {$z_{5:8}$};
\node[goalColor, nodeSize, right= of z1] (zg) {$z_g$};

% Edges
\draw[->, edgeThickness] (s0) -- (s1);
\draw[->, edgeThickness] (s1) -- (s2);
\draw[->, edgeThickness] (s2) -- (s3);
\draw[->, edgeThickness] (s3) -- (s4);
\draw[->, edgeThickness] (s4) -- (s5);
\draw[->, edgeThickness] (s5) -- (s6);
\draw[->, edgeThickness] (s6) -- (s7);
\draw[->, edgeThickness] (s7) -- (s8);

\draw[->, edgeThickness] (a1) -- (s1);
\draw[->, edgeThickness] (a2) -- (s2);
\draw[->, edgeThickness] (a3) -- (s3);
\draw[->, edgeThickness] (a4) -- (s4);
\draw[->, edgeThickness] (a5) -- (s5);
\draw[->, edgeThickness] (a6) -- (s6);
\draw[->, edgeThickness] (a7) -- (s7);
\draw[->, edgeThickness] (a8) -- (s8);

\draw[->, edgeThickness] (s0) -- (a1);
\draw[->, edgeThickness] (s1) -- (a2);
\draw[->, edgeThickness] (s2) -- (a3);
\draw[->, edgeThickness] (s3) -- (a4);
\draw[->, edgeThickness] (s4) -- (a5);
\draw[->, edgeThickness] (s5) -- (a6);
\draw[->, edgeThickness] (s6) -- (a7);
\draw[->, edgeThickness] (s7) -- (a8);

\draw[->, auxiliaryEdgeColor] (z1) -- (a1);
\draw[->, auxiliaryEdgeColor] (z1) -- (a2);
\draw[->, auxiliaryEdgeColor] (z1) -- (a3);
\draw[->, auxiliaryEdgeColor] (z1) -- (a4);

\draw[->, auxiliaryEdgeColor] (z2) -- (a5);
\draw[->, auxiliaryEdgeColor] (z2) -- (a6);
\draw[->, auxiliaryEdgeColor] (z2) -- (a7);
\draw[->, auxiliaryEdgeColor] (z2) -- (a8);

\draw[->, goalEdgeColor] (zg) -- (z1);
\draw[->, goalEdgeColor] (zg) -- (z2);

\draw[->, edgeThickness, bend right=90] (s0) to (z1); % Curved edge
\draw[->, edgeThickness, bend right=90] (s4) to (z2); % Curved edge

\end{tikzpicture}


==> figures/learner.tex <==
\begin{tikzpicture}[
    state/.style={rectangle, draw, minimum height=0.8cm, minimum width=1.4cm, font=\small, align=center, inner sep=0},
    context/.style={fill=Green!20},
    action/.style={fill=Blue!20},
    label/.style={font=\small}
]

% Top part
% \node[state, context] (cthd1) at (0,-2) {$s_{t-h-d-c}$};
\node[state, context] (cthd2) at (1.4,0) {$s_{t-h-c}$};
\node[state, context] (cthd3) at (2.8,0) {...};
\node[state, context] (ctd1) at (4.2,0) {$s_{t-h}$};
\node[state, action] (cd1) at (5.6,0) {$s_{t-h+1}$};
\node[state, action] (cd2) at (7,0) {...};
\node[state, action] (cd3) at (8.4,0) {$s_t$};

\draw[decorate,decoration={brace,amplitude=5pt}] 
    (0.6,0.5) -- (4.9,0.5) node[midway,above,yshift=5pt,label] {Context Length = $c$};

\draw[decorate,decoration={brace,amplitude=5pt}] 
    (4.9,0.5) -- (9.2,0.5) node[midway,above,yshift=5pt,label] {Action Horizon = $h$};

% Bottom part
\node[state, context] (cth1) at (0,-2.2) {$s_{t-h-d-c}$};
\node[state, context] (cth2) at (1.4,-2.2) {...};
\node[state, context] (cth3) at (2.8,-2.2) {$s_{t-h-d}$};
\node[state, action] (ct1) at (4.2,-2.2) {$s_{t-h-d+1}$};
\node[state, action] (ct2) at (5.6,-2.2) {...};
\node[state, action] (ct3) at (7,-2.2) {...};
\node[state, action] (ct4) at (8.4,-2.2) {$s_t$};

\draw[decorate,decoration={brace,amplitude=5pt}] 
    (-0.8,-1.7) -- (3.5,-1.7) node[midway,above,yshift=5pt,label] {Context Length = $c$};

\draw[decorate,decoration={brace,amplitude=5pt}] 
    (3.5,-1.7) -- (9.2,-1.7) node[midway,above,yshift=5pt,label] {Action Horizon = $h+d$};

% Annotations
\draw[<->] (0.0, -2.8) -- (1.5, -2.8) node[right] {\small $d$ more past states};
\draw[<->] (2.9,-0.7) -- (4.2,-0.7) node[right] {\small $d$ more recent states};

\end{tikzpicture}



==> sections/toy.tex <==
\subsection{Diagnostic Simulations} \label{subsec:toy}

\textcolor{red}{Jubayer: need help with writing here (1) how this validates theory (2) significance of problem}

Expert demonstrations often contain sequences of idle actions where the expert stops to think or wait for a change in their environment. A learner must capture the temporal dependencies within the demonstrations since otherwise it could be stuck in an idle state forever. We investigate whether action chunking can help capture these dependencies when the agent's context length is less than that of the expert. In our toy simulations, our state space is $S := \{s_0,s_2,\cdots,s_{10}\}$ where $s_0$ is the starting state and $s_{10}$ is the goal state. Our $(k = 3, 1)-$expert goes right in every state, except in $s_5$ where they are idle unless the states in its memory are $s_5$ i.e $s_{t-1} = s_{t-2} = s_{t=3} = s_5$. We train $(1, h)-$learners, where $h \in \{1, 2, 3, 5\}$, by directly modeling the expert policy distribution from demonstrations. We then count the number of idle actions taken by their learned policy over multiple rollouts. The distribution of idle actions taken in environments with varying stochasticity is shown in Figure \ref{fig:AH_CL_simulation}.

We observe that when the environment is perfectly deterministic, i.e $\delta = 0$ in Proposition 1, larger action horizons almost perfectly capture the expert distribution (which is deterministic) agreeing with Corollary 2. On the other hand, when the environment is highly stochastic, for example with $\delta = 0.90$, an action horizon of 1 outperforms all other learners. With $\delta = 0.40$, there is no discernible, monotonic pattern as to whether the increasing action horizon is better or worse.


\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Sim_noise=0.00.png}
        \label{fig:image1}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Sim_noise=0.40.png}
        \label{fig:image2}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Sim_noise=0.90.png}
        \label{fig:image3}
    \end{minipage}
    \caption{Probability distributions of idle actions taken by learners with varying action horizons in environments with varying stochasticity. Left: environment with noise level 0. Middle: environment with noise = 0.40. Right: environment with noise = 0.90.}
    \label{fig:AH_CL_simulation}
\end{figure}
